HiKonv: High Throughput Quantized Convolution With Novel Bit-wise Management and Computation

Quantization for Convolutional Neural Network (CNN) has shown significant progress with the intention of reducing the cost of computation and storage with low-bitwidth data inputs. There are, however, no systematic studies on how an existing full-bitwidth processing unit, such as CPUs and DSPs, can be better utilized to carry out significantly higher computation throughput for convolution under various quantized bitwidths. In this study, we propose HiKonv, a unified solution that maximizes the compute throughput of a given underlying processing unit to process low-bitwidth quantized data inputs through novel bit-wise parallel computation. We establish theoretical performance bounds using a full-bitwidth multiplier for highly parallelized low-bitwidth convolution, and demonstrate new breakthroughs for high-performance computing in this critical domain. For example, a single 32-bit processing unit can deliver 128 binarized convolution operations (multiplications and additions) under one CPU instruction, and a single 27x18 DSP core can deliver eight convolution operations with 4-bit inputs in one cycle. We demonstrate the effectiveness of HiKonv on CPU and FPGA for both convolutional layers or a complete DNN model. For a convolutional layer quantized to 4-bit, HiKonv achieves a 3.17x latency improvement over the baseline implementation using C++ on CPU. Compared to the DAC-SDC 2020 champion model for FPGA, HiKonv achieves a 2.37x throughput improvement and 2.61x DSP efficiency improvement, respectively.

==> sections/01-introduction.tex <==
\section{Introduction}\label{sec:intro}


Quantization refers to approximating numerical values to lower bitwidths to reduce memory consumption and execution cost~\cite{gholami2021survey}. 
Quantization for deep neural networks (DNN) has gained significant progress, and previous works have proposed numerous quantization methods to reduce the precision of weights, activations, and even gradients while retaining high accuracy~\cite{ul2q, vecq, cong2019dac, zhou2016dorefa}.
Convolution is a popular processing pattern of modern DNNs. It is also known to be multiplication and accumulation (MAC) intensive~\cite{chen2019clouddnn, DNNBuilder, cong2019dac,tdla}.
Quantization makes convolutions more hardware-friendly by leveraging fast, integer-or-logic-only arithmetic units. They replace original high-cost floating-point multiplications with low bitwidth multiplications or even bit-wise operations and reduce memory requirements and bandwidth for data storage and transmission~\cite{ul2q, vecq, chen2019clouddnn, tdla}.

However, the benefit from quantization is limited because the quantized data still utilize high bitwidth arithmetic units for processing and lead to a significant waste of computing resources.
% Given a CPU as the processing platform, 
% the multiplication and accumulation of low bitwidth data would occupy the entire data channel of the underlying Arithmetic Logic Unit (ALU).
% Even with the Single Instruction Multiple Data (SIMD) support, 
For instance, to process a single 4-bit multiplication, a 4-bit data still occupies an 8-bit data width on modern CPUs with AVX support, yet the remaining 4 bits are simply discarded~\cite{AVXforquant}.
% \textcolor{Maroon}{Supporting such low bitwidth data can enable opportunities to boost the throughput of the arithmetic operations significantly, including convolution.}
The waste of the hardware resources for computation becomes more severe when processing the low bitwidth quantized convolution which requires more MAC operations.
This is due to the lack of theoretical support for processing of quantized convolution as well as missing bit-wise management and ignoring the fine-grained computation patterns of the given platform.

% \textcolor{Maroon}{These opportunities also present in reconfigurable hardware platforms.}
Similar drawbacks also happen on the reconfigurable hardware platforms.
Field programmable gate arrays (FPGA) have bit-level configurable flexibility and are manufactured with high precision Digital Signal Processing (DSP) units. 
The flexibility of FPGA enables the DSPs to benefit from SIMD and process more inputs concurrently.
However, without the careful bit-wise management of the input and output, existing solutions only use the given DSPs as multi-channel multipliers and remain a dramatic waste of their computation capacity for quantized convolutions~\cite{xilinxint4, xilinxint8}.
As shown in Figure~\ref{fig:xilinxint4}, the state-of-the-art DSP in a Xilinx FPGA supports parallel processing of two 4-bit multiplicands and two 4-bit multipliers on a single DSP by receiving two multiplicands on two input ports that have internal adder and packing the multipliers in advance to the other port. This solution only provides four concurrent multiplications. 
We can take further advantage of the bit-level management and computation and use the innate computation pattern of the DSPs with careful theoretical deduction to provide many more MAC operations for quantized data in one operation cycle.

\begin{figure}[ht!]
    \centering
    \vspace{-4pt}
    \includegraphics[width=0.45\textwidth]{figures/4channels.png}
    \caption{INT4 optimization on DSP48E2~\cite{xilinxint4}.}
    \vspace{-8pt}
    \label{fig:xilinxint4}
\end{figure}

% I think we are missing some introduction about the computational pattern of the convolution. Basically, our method matches the output of the convolution better while other methods only matches general matrix multiplication.
% \textcolor{Maroon}{To take advantage of all the available bandwidth of a DSP or multiplier and squeeze out their maximum performances}, 
In this paper, we propose HiKonv, a unified solution for accelerating low bitwidth quantized convolution on all platforms.
Specially, we highlight the following contributions:
\begin{itemize}
    % \item We improve input slicing with accurately formulated guard bits that enables the given underlying computing platform to process low bitwidth quantized convolution with maximized concurrency.
    % \item We are the first to use a single multiplier to process multiple sequences of low bitwidth quantized convolutions with novel bit-wise management and computation.
    % \item We further generalize the multiplier-for-convolution solution to support convolutions layers in the DNNs.
    % \item We design a unified formulation to explore the configuration for a given bitwidth to be processed on a given hardware unit. 
    % \item We illustrate HiKonv on CPU platform and achieve upto $3.17\times$ latency improvement for quantized convolution.
    % \item We illustrate HiKonv to DAC-SDC 2020 champion model on FPGA and the on-board result outperforms the throughput and DSP efficiency of the existing champion solution by $2.77\times$ and $3.05\times$, respectively.

    \item We provide three Theorems for using multipliers with high bitwidth inputs to process low bitwidth quantized convolution.
    \item We achieve highest possible throughput for convolution with a single multiplier or DSP for arbitrary bitwidth values with novel bit-wise management and computation.
    \item We further formulate and generalize the technique and construct a highly efficient method to compute convolutional layers with low bitwidth features in DNNs.
    \item CPU implementation of HiKonv achieve up to $3.17 \times$ latency improvement for quantized convolution over conventional methods. 
    \item We illustrate HiKonv to the DAC-SDC 2020 champion model on FPGA. The on-board result outperforms the throughput and DSP efficiency of the champion solution by $2.77 \times$ and $3.05 \times$, respectively. 
    % \item Test cases for demonstration
\end{itemize}

\begin{comment}
This paper is organized as follows: 
We survey the existing software and hardware support for low bitwidth data processing in Section~\ref{sec:backnrelate}.
The preliminaries are introduced in the Section~\ref{sec:prelim}.
Our unified bit grouping solution together with the formulation to find the optimal settings are presented in Section~\ref{sec:formulation}.
Additional implementation optimizations to further improve the efficiency and effectiveness of our solution are presented in Section~\ref{sec:addon}.
We evaluate our solution in Section~\ref{sec:eva}.
Finally, we conclude our paper in the Section~\ref{sec:conclusion}.
\end{comment}

==> sections/03-formulation.tex <==
\section{Formulation}\label{sec:formulation}
% \textcolor{blue}{We first talk about how a multiplication could be segmented, then match the segmented output to a 1d convolution.}

% \textcolor{red}{Add in a figure to present the multiplication of $A$ and $B$, to emphasize the required guard-bit, spacing slice and output.}

\subsection{Input segmentation for multiplication}

Following the bit packing and slicing in the Section~\ref{sec:prelim}, we first look into the situation when multiple data with less bitwidth are packed into the multiplicand and multiplier.

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


Given a length-$N$ vector $f$ and an length-$K$ kernel $g$, where $f$ contains $p$-bit positive integers and $g$ contains $q$-bit positive integers.
Let 
\begin{equation}\label{equ:w}
    W=p+q+\lceil{\log_2max(K,N)}\rceil
\end{equation}
\end{comment}


We construct two new data $A$ and $B$ using the sequences $f$ and $g$ defined in Section~\ref{sec:prelim}, assume both $f$ and $g$ are integer sequences are they are quantized to $p$-bit and $q$-bit, respectively. 
In addition, we define a $W$ which is a constant value when $f$ and $g$ are given:
\begin{equation}
    W=p+q+\lceil{\log_2min(K,N)}\rceil
\end{equation}
$A$ and $B$ are constructed as follows:
\begin{gather}
    % W=p+q+\lceil{\log_2max(K,N)}\rceil\\
    A=\sum_{n=0}^{N-1} f[n]\cdot2^{ W\cdot n }\\
    B=\sum_{k=0}^{K-1} g[k]\cdot 2^{ W\cdot k }
\end{gather}
Naturally, $A$ and $B$ are both integers,
and can be constructed by bit-wise assignment with zero extension function $zext()$:
\begin{gather}
    A[W(n+1)-1:Wn]= zext(f[n])\\
    B[W(k+1)-1:Wk]= zext(g[k])
\end{gather}

The multiplication result $P$ of $A$ and $B$ can be represented as:
\begin{equation}
\begin{split}
    P&=A \times B\\
    &=(\sum_{n=0}^{N-1} f[n]\cdot2^{ W\cdot n })*(\sum_{k=0}^{K-1} g[k]\cdot 2^{ W\cdot k })\\
    &=\sum_{m=0}^{N+K-2} ( \sum_{n+k=m}(f[n]\cdot2^{ W\cdot n }*g[k]\cdot 2^{ W\cdot k }) )\\
    &=\sum_{m=0}^{N+K-2} ( \sum_{n+k=m}(f[n]g[k]\cdot2^{ W\cdot m}))
\end{split}
\end{equation}

% \begin{comment}
\begin{gather}
    p\text{+}(N\text{-}1)*(p\text{+}q\text{+}\lceil{\log_2min(K,N)}\rceil)\leq\log_2A\\
    q\text{+}(K\text{-}1)*(p\text{+}q\text{+}\lceil{\log_2min(K,N)}\rceil)\leq\log_2B
\end{gather}
% \end{comment}



\subsection{Matching to convolution}



\begin{equation}
        P =\sum_{m=0}^{N+K-2} y[m]\cdot2^{ W\cdot m}
\end{equation}

\subsection{Output segmentation}

\subsection{Constructing 3D conv with 1D conv}

==> sections/04-accelerator.tex <==
\section{Further Optimizations towards highest throughput}\label{sec:addon}


\subsection{Output shift and concatenation}

\subsection{Input batching}



As we have mentioned in Section~\ref{sec:back}, the 4-bit quantization has bring us the great opportunity for energy efficiency and performance maintenance.
However, the missing technology on FPGA platform prevent us from enjoying the energy and performance benefit.




Given an 1-D length-$N$ data array $h$ and an length-$K$ filter $f$, we represent the length-$(N\text{+}K\text{-}1)$ output array $y$ of the \textbf{1-D discrete convolution} as $y\text{=}F_{N,K}(h,f)\text{=}h\ast f$. More specifically, the 0-index $m$th element in $y$ can be represent as shown in Equation \ref{eq:1d_conv}. For instance, the output $y$ for 1-D discrete convolution $F_{2,3}$ can be computed as: $[h_0f_0,h_0f_1\text{+}h_1f_0,h_0f_2\text{+}h_1f_1, h_1f_2]$.
\begin{gather}\label{eq:1d_conv}
    y_m=\sum_{k\text{+}n=m}h_nf_k
\end{gather}


In our implementation we focus on the $F_{2,3}$ convolution with $h$ containing 4-bit unsigned integer and $w$ containing 4-bit signed integer. 
We use the embeded MAC operations $Y=A\cdot B\text{+}C$ in Xilinx's DSP48E2 slices to complete the $F_{2,3}$ 1-D discrete convolution. 
In such scenario, the $A$,$B$,$C$, and $Y$ are 27, 18, 45 and 47 bits signed integers. 
We pack $f$ and $h$ into $A$ and $B$ and retrieve the multiplication result $Y$ from the MAC operation as shown in the Equation \ref{eq:pack}.
Since $h$ and $f$ contains only 4-bit integers, the bit width of all the elements in $y$ is less than 10. Then we can represent $Y$ as the sum of elements in $y$ with corresponding trailing zeros and sign bit extensions. The elements of $y$ may be retrieved from $Y$ with equation \ref{eq;unpack}. In such way, each DSP can generate the result of an $F_{2,3}$ 1-D discrete convolution which contains 6 mac operations.

\begin{equation}
\label{eq:pack}
    \begin{split}
        A&= f_2\cdot 2^{22}+f_1\cdot 2^{11}+f_0\\
        B&= h_1\cdot 2^{11}+ h_0\\
        Y&=A\cdot B=2^{33}y_3+2^{22}y_2+2^{11}y_1+y_0
    \end{split}
\end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/SUM_DSPSPLIT.pdf}
    \caption{1-D Discrete Convolution Result from Multiplication}
    \label{fig:sum_split}
\end{figure}
\begin{gather}
\label{eq:unpack}
    y_i=\begin{cases} Y[10:0] &, i=0\\
    Y[11i+10:11i] +zext(y[11i-1])&, i>0
    \end{cases}
\end{gather}

The $F_{2,3}$ 1-D discrete convolution can be extended to $F_{2N,3}$ by addition. 
The extended $F_{2N,3}$ convolution takes a length-$2N$ array $h$ and a length-$3$ filter $f$ as the input and generate an length-$2N\text{+}2$ output array $z$. 
To compute the output array $z$, we first segment array $h$ in to length-$2$ arrays $h^i=[h_{2i},h_{2i+1}]$ and compute the output $y^i=F_{2,3}(h^i,f)$ for each length-2 arrays $h^i$. 
Equation \ref{eq:nd_conv} shows how to compute each element in $z$ with result of $y^i$ in pairs of $z_{2i}$ and $z_{2i+1}$. 
Figure \ref{fig:n_conv} shows the value of  $z_{2i}$ and $z_{2i+1}$ when $i=0$,$i=1$ and $i=N$. 
When $i=0$, $z_{0}=h_0f_0$ and $z_{1}=h_0f_1\text{+}h_1f_0$ according to Equation \ref{eq:1d_conv} which is exactly the value of  $y^0_0$ and $y^0_1$ (colored in blue). 
Similarly, $z_{2N}$ and $z_{2N+1}$ equals $y^{N-1}_3$ and $y^{N-1}_2$ (colored in orange) respectively. 
When $i=1$, $z_{2}$ and $z_{3}$ have three terms, and can be computed by adding up elements in $y^0$ and $y^1$ (colored blue and yellow respectively). 

\begin{gather}
\label{eq:nd_conv}
    [z_{2i},z_{2i+1}]=\begin{cases} 
        [y^{0}_0,y^{0}_1] &, i=0\\
        [y^{N-1}_2,y^{N-1}_3] &, i=N\\
        [y^i_0+y^{i-1}_{2},y^i_1+y^{i-1}_{3}] &, other wise 
    \end{cases}
\end{gather}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/ND_conv.pdf}
    \caption{Computation of $F_{2N,3}$ using $F_{2,3}$}
    \label{fig:n_conv}
\end{figure}

Meanwhile, the computation of 3x3 convolution layer in the neural network can be represented by 










% describe the 1-D convolution algorithm

% describe the 

\subsection{Dataflow construction and latency balancing}
\textcolor{red}{Xinheng, I think the dataflow architecture we are using worth to be presented.}
